LAMM: Language-Assisted Multi-Modal Instruction-Tuning Dataset, Framework, and Benchmark

Large language models have emerged as a promising approach towards achieving general-purpose AI agents. The thriving open-source LLM community has greatly accelerated the development of agents that support human-machine dialogue interaction through natural language processing. However, human interaction with the world extends beyond only text as a modality, and other modalities such as vision are also crucial. Recent works on multi-modal large language models, such as GPT-4V and Bard, have demonstrated their effectiveness in handling visual modalities. However, the transparency of these works is limited and insufficient to support academic research. To the best of our knowledge, we present one of the very first open-source endeavors in the field, LAMM, encompassing a Language-Assisted Multi-Modal instruction tuning dataset, framework, and benchmark. Our aim is to establish LAMM as a growing ecosystem for training and evaluating MLLMs, with a specific focus on facilitating AI agents capable of bridging the gap between ideas and execution, thereby enabling seamless human-AI interaction. Our main contribution is three-fold: 1) We present a comprehensive dataset and benchmark, which cover a wide range of vision tasks for 2D and 3D vision. Extensive experiments validate the effectiveness of our dataset and benchmark. 2) We outline the detailed methodology of constructing multi-modal instruction tuning datasets and benchmarks for MLLMs, enabling rapid scaling and extension of MLLM research to diverse domains, tasks, and modalities. 3) We provide a primary but potential MLLM training framework optimized for modality extension. We also provide baseline models, comprehensive experimental observations, and analysis to accelerate future research. Our baseline model is trained within 24 A100 GPU hours, framework supports training with V100 and RTX3090 is available thanks to the open-source society.

==> sections/10.datasheet.tex <==
% \section*{Datasheet for LAMM Dataset}

\section{Motivation}
\textbf{For what purpose was the dataset created?} Was there a specific task in mind? Was there a specific gap that needed to be filled? Please provide a description. \begin{itemize}
    \item This dataset is created to facilitate research on building large language model. For example, given an image, human can talk with large language model in natural language.
\end{itemize}
\textbf{Who created the dataset (e.g. which team, research group) and on behalf of which entity (e.g. company, institution, organization)?}
\begin{itemize}
    \item This dataset is presented by Shanghai Artificial Intelligence Laboratory, Shanghai AI  Lab in short. Contributors include Zhenfei Yin (Shanghai AI Lab), Jiong Wang (Fudan University), Jianjian Cao (Fudan University), Zhelun Shi (Beihang University), Dingning Li (Dalian University of Technology), Mukai Li (Shanghai AI Lab), Lu Sheng (Beihang University), Xiaoshui Huang (Shanghai AI Lab), Lei Bai (Shanghai AI Lab), Zhiyong Wang (The University of Sydney), Jing Shao(Shanghai AI Lab), Wanli Ouyang (Shanghai AI Lab).
\end{itemize}

\textbf{Who funded the creation of the dataset?} If there is an associated grant, please provide the name of the grantor and the grant name and number.
\begin{itemize}
    \item This work was sponsored by Shanghai Artificial Intelligence Laboratory.
\end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}


\section{Composition}

\textbf{What do the instances that comprise the dataset represent (e.g. documents, photos, people, countries)?} Are there multiple types of instances (e.g., movies, users, and ratings; people and interactions between
them; nodes and edges)? Please provide a description.
\begin{itemize}
    \item There are 186 thousand image-text pairs and 10 thousand point cloud-text pairs for training. Each pair consists of a piece of image/point cloud and corresponding texts. For benchmarking, there are 70 thousand image/point cloud-text pairs covering 14 datasets and 12 tasks.
\end{itemize}

\textbf{How many instances are there in total (of each type, if approciate)?}
\begin{itemize}
    \item For image-instruction pairs, there are 49K samples of n-round daily dialogue, 49k 1-round detailed description, 42K samples of n-round factual knowledge dialogue and 40K samples of 1-round visual task dialogue. Point cloud-instruction pairs consists of 3.3K 1-round visual task dialogue, 2K 1-round detailed description and 4.9K n-round daily dialogue instances.
\end{itemize}

\textbf{Does the dataset contain all possible instances or is it a sample (not necessarily random) of instances from a larger set?} If the dataset is a sample, then what is the larger set? Is the sample representative of the larger set (e.g., geographic coverage)? If so, please describe how this representativeness was validated/verified. If it is not representative of the larger set, please describe why not (e.g., to cover a more diverse range of instances, because instances were withheld or unavailable).
\begin{itemize}
    \item For GPT generated data, we provide all instances obtained. For visual task dialogue data, we select samples from existing dataset and reorganize as instructions by templates we provide. No tests were run to determine representations.
\end{itemize}

\textbf{What data does each instance consist of?} “Raw” data (e.g., unprocessed text or images)or features? In either case, please provide a description.
\begin{itemize}
    \item Each instance consists of the instructions in format of conversations and corresponding image or point cloud.
\end{itemize}

\textbf{Is there a label or target associated with each instance?} If so, please provide a description.
\begin{itemize}
    \item The label is response of assistant in instructions.
\end{itemize}

\textbf{Is any information missing from individual instances?} If so, please provide a description, explaining why this information is missing (e.g., because it was unavailable). This does not include intentionally removed information, but might include, e.g. redacted text.
\begin{itemize}
    \item Everything is included.
\end{itemize}

\textbf{Are relationships between individual instances made explicit (e.g. users' movie ratings, social network links)?} If so, please describe how these relationships are made explicit.
\begin{itemize}
    \item Each instance is labeled by corresponding task type.
\end{itemize}

\textbf{Are there recommended data splits (e.g., training, development/validation, testing)?} If so, please provide a description of these splits, explaining the rationale behind them.
\begin{itemize}
    \item The instances are divided into training set and test set. No dataset sharing between training and testing set for zero-shot setting in our benchmark.
\end{itemize}

\textbf{Are there any errors, sources of noise, or redundancies in the dataset?} If so, please provide a description.
\begin{itemize}
    \item For instructions generated by GPT-API, instructions may not cover all information in image/point cloud accurately because the GPT-API cannot accept visual content directly.
\end{itemize}

\textbf{Is the dataset self-contained, or does it link to or otherwise rely on external resources (e.g. websites, tweets, other datasets)?} If it links to or relies on external resources, a) are there guarantees that they will exist, and remain constant, over time; b) are there official archival versions of the complete dataset (i.e., including the external resources as they existed at the time the dataset was created); c) are there any restrictions (e.g., licenses, fees) associated with any of the external resources that might apply to a dataset consumer? Please provide descriptions of all external resources and any restrictions associated with them, as well as links or other access points, as appropriate.
\begin{itemize}
    \item The dataset is entirely self-contained.
\end{itemize}

\textbf{Does the dataset contain data that might be considered confidential (e.g. data that is protected by legal privilege or by doctor-patient confidentially, data that includes the content of individuals' non-public communications)?} If so, please provide a description.
\begin{itemize}
    \item No. All data leveraged in dataset construction are publicly available or from public tools (e.g. GPT-API).
\end{itemize}

\textbf{Does the dataset contain data that, if viewed directly, might be offensive, insulting, threatening, or might otherwise cause anxiety?} If so, please describe why.
\begin{itemize}
    \item Instructions generated by GPT-API may contain some inappropriate messages due to its bias. We briefly filtered data in order to minimize such occurrences as much as possible.
\end{itemize}

\textbf{Does the dataset identify any subpopulations (e.g. by age, gender)?} If so, please describe how these subpopulations are identified and provide a description of their respective distributions within the dataset.
\begin{itemize}
    \item No.
\end{itemize}

\textbf{Is it possible to identify individuals (i.e., one or more natural persons), either directly or indirectly (i.e., in combination with other
data) from the dataset?} If so, please describe how.
\begin{itemize}
    \item Some human images are included in this dataset but they should be anonymous.
\end{itemize}

\textbf{Does the dataset contain data that might be considered sensitive in any way (e.g., data that reveals race or ethnic origins, sexual orientations, religious beliefs, political opinions or union memberships, or locations; financial or health data; biometric or genetic data; forms of government identification, such as social security numbers; criminal history)?} If so, please provide a description.
\begin{itemize}
    \item No. 
\end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No. 
\end{itemize}


\section{Collection Process}

\textbf{How was the data associated with each instance acquired?}  Was the
data directly observable (e.g., raw text, movie ratings), reported by subjects (e.g., survey responses), or indirectly inferred/derived from other data (e.g., part-of-speech tags, model-based guesses for age or language)? If the data was reported by subjects or indirectly inferred/derived from other data, was the data validated/verified? If so, please describe how.
\begin{itemize}
    \item Data was observable as raw text, images or point cloud. Images and point cloud are selected from existing public vision dataset, while instructions are either fully generated by ChatGPT or reorganized by template from ChatGPT.
\end{itemize}

\textbf{What mechanisms or procedures were used to collect data (e.g. hardware apparatuses or sensors, manual human curation, software programs, software APIS)?} How were these mechanisms or procedures validated?
\begin{itemize}
    \item Instructions and templates are obtained by ChatGPT API. Part of data are manual confirmed.
\end{itemize}

\textbf{If the dataset is a sample from a larger set, what was the sampling strategy (e.g. deterministic, probabilistic with specific sampling probabilities)?}
\begin{itemize}
    \item For images from large-scale datasets such COCO \cite{coco2014} and Bamboo \cite{zhang2022bamboo}, instances are randomly selected. For items from small datasets, all instances are adopted.
\end{itemize}

\textbf{Who was involved in the data collection process (e.g. students, crowdworkers, contractors) and how were they compensated (e.g. how much were crowdworkers paid)?}
\begin{itemize}
    \item Data collection process is fully conducted by authors.
\end{itemize}


\textbf{Over what timeframes was the data collected?} Does this timeframe match the creation timeframe of the data associated with the instances (e.g., recent crawl of old news articles)? If not, please describe the timeframe in which the data associated with the instances was created.
\begin{itemize}
    \item Our dataset is collected in May 2023. No instance is associated with timeframe.
\end{itemize}

% \textbf{Were any ethical review processes conducted (e.g. by an institutional review board)?}  If so, please provide a description of these review processes, including the outcomes, as well as a link or other access point to any supporting documentation.
% \begin{itemize}
%     \item N/A
% \end{itemize}

% \textbf{Did you collect the data from the individuals in question directly, or obtain it via third parties or other sources (e.g., websites)?} 
% \begin{itemize}
%     \item N/A
% \end{itemize}

% \textbf{Were the individuals in question notified about the data collection?} If so, please describe (or show with screenshots or other information) how
% notice was provided, and provide a link or other access point to, or otherwise reproduce, the exact language of the notification itself.
% \begin{itemize}
%     \item N/A
% \end{itemize}

% \textbf{Did the individuals in question consent to the collection and use of their data?} If so, please describe (or show with screenshots or other
% information) how consent was requested and provided, and provide a link
% or other access point to, or otherwise reproduce, the exact language to
% which the individuals consented.
% \begin{itemize}
%     \item N/A
% \end{itemize}

% \textbf{If consent was obtained, were the consenting individuals provided with a mechanism to revoke their consent in the future or for certain uses?} If so, please provide a description, as well as a link or other access
% point to the mechanism (if appropriate).
% \begin{itemize}
%     \item N/A
% \end{itemize}

% \textbf{Has an analysis of the potential impact of the dataset and its use on data subjects (e.g., a data protection impact analysis) been conducted?}  If so, please provide a description of this analysis, including the
% outcomes, as well as a link or other access point to any supporting documentation.
% \begin{itemize}
%     \item N/A
% \end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}



\section{Preprocessing/cleaning/labeling}

\textbf{Was any preprocessing/cleaning/labeling of the data done (e.g., discretization or bucketing, tokenization, part-of-speech tagging, SIFT feature extraction, removal of instances, processing of missing values)?} If so, please provide a description. If not, you may skip the remaining questions in this section.
\begin{itemize}
    \item Texts generated by GPT-API of incorrect format are removed in preprocessing.
\end{itemize}

\textbf{Was the “raw” data saved in addition to the preprocessed/cleaned/labeled data (e.g., to support unanticipated future uses)?} If so, please provide a link or other access point to the
“raw” data.
\begin{itemize}
    \item Yes, source dataset and original file names are saved.
\end{itemize}

\textbf{Is the software that was used to preprocess/clean/label the data available?} If so, please provide a link or other access point.
\begin{itemize}
    \item Yes, GPT-API for instruction and template generation is available on \url{https://openai.com/chatgpt}.
\end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}


\section{Uses}

\textbf{Has the dataset been used for any tasks already?} If so, please provide a description.
\begin{itemize}
    \item At the time of publication, the data has been used for multimodal large language model instruction tuning and relative performance evaluation.
\end{itemize}

\textbf{Is there a repository that links to any or all papers or systems that use the dataset?} If so, please provide a link or other access point.
\begin{itemize}
    \item There is a repository at \url{https://github.com/BradyFU/Awesome-Multimodal-Large-Language-Models} containing some papers used the dataset.
\end{itemize}

\textbf{What (other) tasks could the dataset be used for?}
\begin{itemize}
    \item The dataset could be used for image generation or image captioning.
\end{itemize}

% \textbf{Is there anything about the composition of the dataset or the way it was collected and preprocessed/cleaned/labeled that might impact future uses?} For example, is there anything that a dataset consumer might need to know to avoid uses that could result in unfair treatment of individuals or groups (e.g., stereotyping, quality of service issues) or other risks or harms (e.g., legal risks, financial harms)? If so, please provide a description. Is there anything a dataset consumer could do to mitigate these risks or harms?
% \begin{itemize}
%     \item No. 
% \end{itemize}

% \textbf{Are there tasks for which the dataset should not be used?} If so, please provide a description.
% \begin{itemize}
%     \item No.
% \end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}

\section{Distribution}

\textbf{Will the dataset be distributed to third parties outside of the entity (e.g., company, institution, organization) on behalf of which the dataset was created?} If so, please provide a description.
\begin{itemize}
    \item Yes, the dataset is publicly available.
\end{itemize}

\textbf{How will the dataset will be distributed (e.g., tarball on website, API,
GitHub)?} Does the dataset have a digital object identifier (DOI)?
\begin{itemize}
    \item The dataset is distributed on Huggingface (\url{https://huggingface.co/datasets/openlamm/LAMM_Dataset/tree/main}) and OpenDataLab (\url{https://opendatalab.com/LAMM/LAMM}). No DOI for the dataset.
\end{itemize}

\textbf{When will the dataset be distributed?}
\begin{itemize}
    \item The dataset was released in June 2023.
\end{itemize}

\textbf{Will the dataset be distributed under a copyright or other intellectual property (IP) license, and/or under applicable terms of use (ToU)?} If so, please describe this license and/or ToU, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms or ToU, as well as any fees associated with these restrictions.
\begin{itemize}
    \item The dataset is publicly available under license of Creative Commons licenses (CC-BY) if no special state for source datasets.
\end{itemize}

% \textbf{Have any third parties imposed IP-based or other restrictions on the data associated with the instances?} If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any relevant licensing terms, as well as any fees associated with these restrictions.
% \begin{itemize}
%     \item No.
% \end{itemize}

% \textbf{Do any export controls or other regulatory restrictions apply to the dataset or to individual instances?} If so, please describe these restrictions, and provide a link or other access point to, or otherwise reproduce, any supporting documentation.
% \begin{itemize}
%     \item No.
% \end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}


\section{Maintenance}

\textbf{Who will be supporting/hosting/maintaining the dataset?}
\begin{itemize}
    \item The dataset is supporting/maintaining by Jiong Wang and Zhelun Shi.
\end{itemize}

\textbf{How can the owner/curator/manager of the dataset be contacted
(e.g., email address)?}
\begin{itemize}
    \item The curators, Zhenfei Yin, Lei Bai and Jing Shao, can be contacted at \url{{yinzhenfei, bailei, shaojing}@pjlab.org.cn}.
\end{itemize}

\textbf{Is there an erratum?} If so, please provide a link or other access point.
\begin{itemize}
    \item No.
\end{itemize}

\textbf{Will the dataset be updated (e.g., to correct labeling errors, add new
instances, delete instances)?} If so, please describe how often, by
whom, and how updates will be communicated to dataset consumers (e.g.,
mailing list, GitHub)?
\begin{itemize}
    \item Updates of the dataset will be posted at Github page (\url{https://github.com/OpenLAMM/LAMM}) and project page (\url{https://openlamm.github.io}).
\end{itemize}


% \textbf{If the dataset relates to people, are there applicable limits on the retention of the data associated with the instances (e.g., were the individuals in question told that their data would be retained for a fixed
% period of time and then deleted)?} If so, please describe these limits and
% explain how they will be enforced.
% \begin{itemize}
%     \item N/A.
% \end{itemize}


% \textbf{Will older versions of the dataset continue to be supported/hosted/maintained?} If so, please describe how. If not, please describe how its obsolescence will be communicated to dataset consumers.
% \begin{itemize}
%     \item N/A.
% \end{itemize}

\textbf{If others want to extend/augment/build on/contribute to the dataset, is there a mechanism for them to do so?} If so, please provide a description. Will these contributions be validated/verified? If so, please describe how. If not, why not? Is there a process for communicating/distributing these contributions to dataset consumers? If so, please provide a description.
\begin{itemize}
    \item Yes, contributions to our dataset are welcomed. These contributions can be raised in huggingface community and commited after manual review.
\end{itemize}

\textbf{Any other comments?}
\begin{itemize}
    \item No.
\end{itemize}


==> sections/9.checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerNo{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

